In Defense of Lazy Visual Grounding for Open-Vocabulary Semantic Segmentation

We present lazy visual grounding, a two-stage approach of unsupervised object mask discovery followed by object grounding, for open-vocabulary semantic segmentation. Plenty of the previous art casts this task as pixel-to-text classification without object-level comprehension, leveraging the image-to-text classification capability of pretrained vision-and-language models. We argue that visual objects are distinguishable without the prior text information as segmentation is essentially a vision task. Lazy visual grounding first discovers object masks covering an image with iterative Normalized cuts and then later assigns text on the discovered objects in a late interaction manner. Our model requires no additional training yet shows great performance on five public datasets: Pascal VOC, Pascal Context, COCO-object, COCO-stuff, and ADE 20K. Especially, the visually appealing segmentation results demonstrate the model capability to localize objects precisely. Paper homepage: https://cvlab.postech.ac.kr/research/lazygrounding

==> asset/main/table/backbone.tex <==




==> asset/main/table/bgfg.tex <==




\begin{table*}[t!]
    \centering
    \caption{Ablation study of the background post-processing}
    \tabcolsep=0.1cm
    \scalebox{0.85}{
    \begin{tabular}{clll}
    \toprule
    background post-processing & VOC21 & Context60 & COCO-Object \\\midrule
     & 60.3 & 34.8 & \\ 
    \rowcolor{gray!10}
    $\checkmark$ (ours) & 61.7 (+1.4) &  &  \\ \bottomrule
    \end{tabular}
    }
    \label{table:bgfg}
\end{table*}
